Neutron and proton electric dipole moments from $N_f=2+1$ domain-wall fermion lattice QCD

We present a lattice calculation of the neutron and proton electric dipole moments (EDM's) with $N_f=2+1$ flavors of domain-wall fermions. The neutron and proton EDM form factors are extracted from three-point functions at the next-to-leading order in the $\theta$ vacuum of QCD. In this computation, we use pion masses 0.33 and 0.42 GeV and 2.7 fm$^3$ lattices with Iwasaki gauge action and a 0.17 GeV pion and 4.6 fm$^3$ lattice with I-DSDR gauge action, all generated by the RBC and UKQCD collaborations. The all-mode-averaging technique enables an efficient and high statistics calculation. Chiral behavior of lattice EDM's is discussed in the context of baryon chiral perturbation theory. In addition, we also show numerical evidence on relationship of three- and two-point correlation function with local topological distribution.

==> table_gem_m0.001_ID.tex <==
\begin{table}
\begin{center}
\caption{Same as Tab.~\ref{tab:gem_m0.005} but for I-DSDR 32$^3$, 170 MeV pion ensemble.}
\label{tab:gem_m0.001ID}
\begin{tabular}{ccccc}
\hline\hline
 & & $t_{\rm sep}=1.3$ fm\\
\hline
  & P & & N\\
\hline
fit-range & $[  3,   6]$ & $[  3,   6]$ & $[  3,   6]$ & $[  3,   6]$ \\
\hline
$q^2$(GeV$^2$) & $G_e^p$ & $G_m^p$ & $G_e^n$ & $G_m^n$ \\
 0.072&   0.830( 8)&   2.177(100)&  -0.001( 3)&  -1.240(71)\\
 0.141&   0.713( 9)&   1.900(72)&   0.009( 4)&  -1.125(57)\\
 0.208&   0.623(13)&   1.659(81)&   0.013( 6)&  -0.956(63)\\
 0.273&   0.564(12)&   1.498(79)&   0.017( 9)&  -0.841(64)\\
\hline\hline
\end{tabular}
\end{center}
\end{table}


==> table_gem_m0.005.tex <==
\begin{table}
\begin{center}
\caption{The electric and magnetic form factors for the neutron (N) and proton (P). 
Iwasaki 24$^3$, 330 MeV pion ensemble. [] denotes fit range.
}\label{tab:gem_m0.005}
\begin{tabular}{ccccc|cccc}
\hline\hline
 & & $t_{\rm sep}=1.32$ fm & & & & $t_{\rm sep}=0.9$ fm\\
\hline
  & P & & N & & P & & N\\
\hline
fit-range & $[  4,   8]$ & $[  4,   8]$ & $[  4,   8]$ & $[  4,   8]$ 
          & $[  3,   5]$ & $[  3,   5]$ & $[  3,   5]$ & $[  3,   5]$ \\
\hline
$q^2$(GeV$^2$) & $G_e^p$ & $G_m^p$& $G_e^n$ & $G_m^n$ & 
                 $G_e^p$ & $G_m^p$& $G_e^n$ & $G_m^n$\\
 0.210&   0.715( 5)&   1.927(36)&   0.012( 2)&  -1.186(25)&
 0.712( 2)&   1.846(19)&   0.016( 1)&  -1.153(13)\\
 0.405&   0.555( 6)&   1.515(29)&   0.019( 3)&  -0.946(20)&
 0.545( 2)&   1.472(16)&   0.023( 1)&  -0.923(11)\\
 0.586&   0.432( 9)&   1.210(36)&   0.030( 5)&  -0.768(26)&
 0.435( 4)&   1.219(18)&   0.025( 2)&  -0.772(12)\\
 0.760&   0.339(13)&   0.995(50)&   0.027( 8)&  -0.601(33)&
 0.366( 5)&   1.020(23)&   0.029( 2)&  -0.623(15)\\
\hline\hline
\end{tabular}
\end{center}
\end{table}


==> table_gem_m0.01.tex <==
\begin{table}
\begin{center}
\caption{Same as Tab.~\ref{tab:gem_m0.005} but for 420 MeV pion.}
\label{tab:gem_m0.01}
\begin{tabular}{ccccc|cccc}
\hline\hline
 & &$t_{\rm sep}=1.32$ fm & & & & $t_{\rm sep}=0.9$ fm\\
\hline
  & P & & N & & P & & N\\
\hline
fit-range & $[  4,   8]$ & $[  4,   8]$ & $[  4,   8]$ & $[  4,   8]$ 
          & $[  3,   5]$ & $[  3,   5]$ & $[  3,   5]$ & $[  3,   5]$ \\
\hline
$q^2$(GeV$^2$) & $G_e^p$ & $G_m^p$ & $G_e^n$ & $G_m^n$ &
                 $G_e^p$ & $G_m^p$& $G_e^n$ & $G_m^n$\\
 0.199&   0.731( 4)&   1.974(27)&   0.012( 2)&  -1.218(19)&
 0.738( 2)&   1.881(19)&   0.012( 1)&  -1.176(12)\\
 0.387&   0.573( 4)&   1.573(24)&   0.013( 2)&  -0.968(16)&
 0.575( 2)&   1.507(17)&   0.017( 1)&  -0.945(11)\\
 0.568&   0.464( 6)&   1.294(27)&   0.013( 4)&  -0.777(19)&
 0.466( 3)&   1.253(16)&   0.018( 1)&  -0.783(11)\\
 0.735&   0.388( 9)&   1.109(38)&   0.020( 6)&  -0.680(25)&
 0.387( 5)&   1.042(18)&   0.023( 2)&  -0.654(12)\\
\hline\hline
\end{tabular}
\end{center}
\end{table}

